CUORE Opens the Door to Tonne-scale Cryogenics Experiments

The past few decades have seen major developments in the design and operation of cryogenic particle detectors. This technology offers an extremely good energy resolution - comparable to semiconductor detectors - and a wide choice of target materials, making low temperature calorimetric detectors ideal for a variety of particle physics applications. Rare event searches have continued to require ever greater exposures, which has driven them to ever larger cryogenic detectors, with the CUORE experiment being the first to reach a tonne-scale, mK-cooled, experimental mass. CUORE, designed to search for neutrinoless double beta decay, has been operational since 2017 at a temperature of about 10 mK. This result has been attained by the use of an unprecedentedly large cryogenic infrastructure called the CUORE cryostat: conceived, designed and commissioned for this purpose. In this article the main characteristics and features of the cryogenic facility developed for the CUORE experiment are highlighted. A brief introduction of the evolution of the field and of the past cryogenic facilities are given. The motivation behind the design and development of the CUORE cryogenic facility is detailed as are the steps taken toward realization, commissioning, and operation of the CUORE cryostat. The major challenges overcome by the collaboration and the solutions implemented throughout the building of the cryogenic facility will be discussed along with the potential improvements for future facilities. The success of CUORE has opened the door to a new generation of large-scale cryogenic facilities in numerous fields of science. Broader implications of the incredible feat achieved by the CUORE collaboration on the future cryogenic facilities in various fields ranging from neutrino and dark matter experiments to quantum computing will be examined.

==> CUORE - PPNP_arXiv/cuore-authors.tex <==
% Updated on Friday, 16 Aug 2021 + PRL 2018 + Tech 
\author[USC]{D.~Q.~Adams}
\author[USC]{C.~Alduino}
\author[INFNMilano]{F.~Alessandria\fnref{fn2}}
\author[UCLA]{K.~Alfonso}
\author[Como,INFNMiB]{E.~Andreotti}
\author[USC]{F.~T.~Avignone~III}
\author[INFNLegnaro]{O.~Azzolini}
\author[LNGS]{M.~Balata}
\author[USC]{I.~Bandac}
\author[BerkeleyPhys,LBNLNucSci]{T.~I.~Banks}
\author[INFNBologna]{G.~Bari}
\author[Firenze,INFNFirenze]{M.~Barucci}
\author[LBNLMater]{J.~W.~Beeman\fnref{fn2}}
\author[Roma,INFNRoma]{F.~Bellini}
\author[LNGS]{G.~Benato}
\author[BerkeleyPhys]{M.~Beretta}
\author[INFNGenova]{A.~Bersani}
\author[LBNLNucSci]{D.~Biare}
\author[INFNMiB]{M.~Biassoni}
\author[INFNGenova]{F.~Bragazzi}
\author[Milano,INFNMiB]{A.~Branca}
\author[Milano,INFNMiB]{C.~Brofferio}
\author[LBNLNucSci,BerkeleyPhys]{A.~Bryant}
\author[INFNRoma]{A.~Buccheri\fnref{fn2}}
\author[LNGS]{C.~Bucci}
\author[INFNRoma]{C.~Bulfon}
\author[INFNLegnaro]{A.~Camacho}
\author[VirginiaTech]{J.~Camilleri}
\author[INFNGenova]{A.~Caminata}
\author[Genova,INFNGenova]{A.~Campani}
\author[MIT,LNGS]{L.~Canonica}
\author[Fudan]{X.~G.~Cao}
\author[Milano,INFNMiB]{S.~Capelli}
\author[INFNRoma]{M.~Capodiferro}
\author[LNGS,BerkeleyPhys,LBNLNucSci]{L.~Cappelli}
\author[INFNRoma]{L.~Cardani}
\author[INFNGenova]{M.~Cariello}
\author[Milano,INFNMiB]{P.~Carniti}
\author[Milano,INFNMiB]{M.~Carrettoni}
\author[INFNRoma]{N.~Casali}
\author[Milano,INFNMiB]{L.~Cassina}
\author[GSSI,LNGS]{E.~Celi}
\author[INFNGenova]{R.~Cereseto}
\author[INFNMiB]{G.~Ceruti}
\author[INFNBologna]{A.~Chiarini}
\author[Milano,INFNMiB]{D.~Chiesa}
\author[USC]{N.~Chott}
\author[Milano,INFNMiB]{M.~Clemenza}
\author[INFNLegnaro]{D.~Conventi}
\author[Genova,INFNGenova]{S.~Copello}
\author[Roma,INFNRoma]{C.~Cosmelli}
\author[INFNMiB]{O.~Cremonesi}
\author[INFNBologna]{C.~Crescentini}
\author[USC]{R.~J.~Creswick}
\author[Yale]{J.~S.~Cushman}
\author[GSSI,LNGS]{A.~D'Addabbo}
\author[LNGS,Cassino]{D.~D'Aguanno}
\author[INFNRoma]{I.~Dafinei}
\author[INFNMiB]{V.~Datskov}
\author[Yale]{C.~J.~Davis}
\author[INFNBologna]{F.~Del Corso}
\author[Milano,INFNMiB]{S.~Dell'Oro}
\author[BolognaAstro,INFNBologna]{M.~M.~Deninno\fnref{fn1}}
\author[Genova,INFNGenova]{S.~Di~Domizio}
\author[GSSI,LNGS]{V.~Domp\`{e}}
\author[LNGS,AQUILA]{M.~L.~Di Vacri}
\author[LNGS]{L.~Di Paolo}
\author[BerkeleyPhys,LBNLNucSci]{A.~Drobizhev}
\author[WISC]{L.~Ejzak}
\author[Roma,INFNRoma]{R.~Faccini}
\author[Fudan]{D.~Q.~Fang}
\author[Roma,INFNRoma]{G.~Fantini}
\author[Milano,INFNMiB]{M.~Faverzani}
\author[Milano,INFNMiB]{E.~Ferri}
\author[GSSI,INFNRoma]{F.~Ferroni}
\author[INFNMiB,Milano]{E.~Fiorini}
\author[INFNFrascati]{M.~A.~Franceschi}
\author[LBNLNucSci,BerkeleyPhys]{S.~J.~Freedman\fnref{fn1}}
\author[Fudan]{S.~H.~Fu}
\author[LBNLNucSci]{B.~K.~Fujikawa}
\author[INFNMiB]{R.~Gaigher}
\author[GSSI,LNGS]{S.~Ghislandi}
\author[Milano,INFNMiB]{A.~Giachero}
\author[Milano,INFNMiB]{L.~Gironi}
\author[Paris-Saclay]{A.~Giuliani}
\author[MIT]{L.~Gladstone}
\author[LNGS]{J.~Goett}
\author[LNGS]{P.~Gorla}
\author[INFNMiB]{C.~Gotti}
\author[INFNBologna]{C.~Guandalini}
\author[INFNBologna]{M.~Guerzoni}
\author[LNGS]{M.~Guetti}
\author[CalPoly]{T.~D.~Gutierrez}
\author[LBNLMater,MatBerkely]{E.~E.~Haller\fnref{fn1}}
\author[SJTU]{K.~Han}
\author[BerkeleyPhys]{E.~V.~Hansen}
\author[Yale]{K.~M.~Heeger}
\author[BerkeleyPhys,LBNLNucSci]{R.~Hennings-Yeomans}
\author[UCLA]{K.~P.~Hickerson}
\author[BerkeleyPhys]{R.~G.~Huang}
\author[UCLA]{H.~Z.~Huang}
\author[INFNRoma]{M.~Iannone}
\author[LNGS]{L.~Ioannucci}
\author[MIT]{J.~Johnston}
\author[LBNLPhys]{R.~Kadel\fnref{fn2}}
\author[INFNLegnaro]{G.~Keppel}
\author[LBNLNucSci,BerkeleyPhys]{L.~Kogler}
\author[BerkeleyPhys,LBNLNucSci]{Yu.~G.~Kolomensky}
\author[MIT]{A.~Leder}
\author[INFNFrascati]{C.~Ligi}
\author[Yale]{K.~E.~Lim}
\author[Yale]{R.~Liu}
\author[UCLA]{L.~Ma}
\author[Fudan]{Y.~G.~Ma}
\author[Milano,INFNMiB]{C.~Maiano}
\author[Milano]{M.~Maino}
\author[GSSI,LNGS]{L.~Marini}
\author[UNIZA,ARAID]{M.~Martinez}
\author[USC]{C.~Martinez Amaya}
\author[Yale]{R.~H.~Maruyama}
\author[MIT]{D.~Mayer}
\author[INFNMiB]{R.~Mazza}
\author[LBNLNucSci]{Y.~Mei}
\author[BolognaAstro,INFNBologna]{N.~Moggi}
\author[INFNRoma]{S.~Morganti}
\author[INFNRoma]{P.~J.~Mosteiro}
\author[LNGS,GSSI]{S.~S.~Nagorny}
\author[INFNFrascati]{T.~Napolitano}
\author[Milano,INFNMiB]{M.~Nastasi}
\author[Yale]{J.~Nikkel}
\author[LNGS]{S.~Nisi}
\author[Saclay]{C.~Nones}
\author[LLNL,BerkeleyNucEng]{E.~B.~Norman}
\author[Paris-Saclay]{V.~Novati}
\author[Milano,INFNMiB]{A.~Nucciotti}
\author[Milano,INFNMiB]{I.~Nutini}
\author[VirginiaTech]{T.~O'Donnell}
\author[INFNGenova]{M.~Olcese}
\author[Firenze,INFNFirenze]{E.~Olivieri}
\author[INFNRoma]{F.~Orio}
\author[LNGS]{D.~Orlandi}
\author[MIT]{J.~L.~Ouellet}
\author[Yale]{S.~Pagan}
\author[LNGS,Cassino]{C.~E.~Pagliarone}
\author[GSSI,LNGS]{L.~Pagnanini}
\author[Genova,INFNGenova]{M.~Pallavicini}
\author[INFNLegnaro]{V.~Palmieri\fnref{fn1}}
\author[LNGS]{L.~Pattavina}
\author[Milano,INFNMiB]{M.~Pavan}
\author[LLNL]{M.~Pedretti}
\author[INFNPadova]{R.~Pedrotta}
\author[INFNRoma]{A.~Pelosi}
\author[INFNMiB]{M.~Perego}
\author[INFNMiB]{G.~Pessina}
\author[INFNRoma]{V.~Pettinacci}
\author[INFNRoma]{G.~Piperno}
\author[INFNLegnaro]{C.~Pira}
\author[LNGS]{S.~Pirro}
\author[Milano,INFNMiB]{S.~Pozzi}
\author[Milano,INFNMiB]{E.~Previtali}
\author[GSSI,LNGS]{A.~Puiu}
\author[GSSI,LNGS]{S.~Quitadamo}
\author[INFNRoma]{F.~Reindl}
\author[BolognaAstro,INFNBologna]{F.~Rimondi\fnref{fn1}}
\author[Firenze,INFNFirenze]{L.~Risegari}
\author[USC]{C.~Rosenfeld}
\author[INFNGenova]{C.~Rossi}
\author[USC,LNGS]{C.~Rusconi}
\author[BerkeleyPhys]{M.~Sakai}
\author[Milano,INFNMiB]{E.~Sala}
\author[Como,INFNMiB]{C.~Salvioni}
\author[LLNL]{S.~Sangiorgio}
\author[LNGS,AQUILA]{D.~Santone}
\author[Milano,INFNMiB]{D.~Schaeffer}
\author[LBNLNucSci]{B.~Schmidt}
\author[UCLA]{J.~Schmidt}
\author[LLNL]{N.~D.~Scielzo}
\author[VirginiaTech]{V.~Sharma}
\author[BerkeleyPhys]{V.~Singh}
\author[INFNMiB]{M.~Sisti}
\author[LBNLNucSci]{A.~R.~Smith\fnref{fn1}}
\author[JHU]{D.~Speller}
\author[INFNLegnaro]{F.~Stivanello}
\author[Yale]{P.~T.~Surukuchi}
\author[INFNPadova]{L.~Taffarello}
\author[LNGS]{L.~Tatananni}
\author[Paris-Saclay]{M.~Tenconi}
\author[Milano,INFNMiB]{F.~Terranova}
\author[INFNPadova]{M.~Tessaro}
\author[INFNRoma]{C.~Tomei}
\author[Firenze,INFNFirenze]{G.~Ventura}
\author[BerkeleyPhys,LBNLNucSci]{K.~J.~Vetter}
\author[Roma,INFNRoma]{M.~Vignati}
\author[BerkeleyPhys,LBNLNucSci]{S.~L.~Wagaarachchi}
\author[LBNLEngineering]{J.~Wallig}
\author[LLNL,BerkeleyNucEng]{B.~S.~Wang}
\author[Fudan]{H.~W.~Wang}
\author[LBNLNucSci]{B.~Welliver}
\author[USC]{J.~Wilson}
\author[USC]{K.~Wilson}
\author[MIT]{L.~A.~Winslow}
\author[Yale,WISC]{T.~Wise\fnref{fn2}}
\author[Milano,INFNMiB]{L.~Zanotti\fnref{fn2}}
\author[LNGS]{C.~Zarra}
\author[Fudan]{G.~Q.~Zhang}
\author[UCLA]{B.~X.~Zhu}
\author[LBNLEngineering]{S.~Zimmermann}
\author[BolognaAstro,INFNBologna]{S.~Zucchelli}

\address[USC]{Department of Physics and Astronomy, University of South Carolina, Columbia, SC 29208, USA}
\address[INFNMilano]{INFN -- Sezione di Milano, Milano I-20133, Italy}
\address[UCLA]{Department of Physics and Astronomy, University of California, Los Angeles, CA 90095, USA}
\address[Como]{Dipartimento di Fisica e Matematica, Universit\`{a} dell’Insubria, Como I-22100, Italy}
\address[INFNMiB]{INFN -- Sezione di Milano Bicocca, Milano I-20126, Italy}
\address[Milano]{Dipartimento di Fisica, Universit\`{a} di Milano-Bicocca, Milano I-20126, Italy}
\address[INFNLegnaro]{INFN -- Laboratori Nazionali di Legnaro, Legnaro (Padova) I-35020, Italy}
\address[INFNBologna]{INFN -- Sezione di Bologna, Bologna I-40127, Italy}
\address[Firenze]{Dipartimento di Fisica, Universit\`{a} di Firenze, Firenze I-50125, Italy}
\address[INFNFirenze]{INFN -- Sezione di Firenze, Firenze I-50125, Italy}
\address[LBNLMater]{Materials Science Division, Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\address[Roma]{Dipartimento di Fisica, Sapienza Universit\`{a} di Roma, Roma I-00185, Italy}
\address[INFNRoma]{INFN -- Sezione di Roma, Roma I-00185, Italy}
\address[LNGS]{INFN -- Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila) I-67100, Italy}
\address[BerkeleyPhys]{Department of Physics, University of California, Berkeley, CA 94720, USA}
\address[VirginiaTech]{Center for Neutrino Physics, Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061, USA}
\address[INFNGenova]{INFN -- Sezione di Genova, Genova I-16146, Italy}
\address[Genova]{Dipartimento di Fisica, Universit\`{a} di Genova, Genova I-16146, Italy}
\address[MIT]{Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\address[Fudan]{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE), Institute of Modern Physics, Fudan University, Shanghai 200433, China}
\address[LBNLNucSci]{Nuclear Science Division, Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}
\address[GSSI]{Gran Sasso Science Institute, L'Aquila I-67100, Italy}
\address[INFNFrascati]{INFN -- Laboratori Nazionali di Frascati, Frascati (Roma) I-00044, Italy}
\address[Paris-Saclay]{Université Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\address[CalPoly]{Physics Department, California Polytechnic State University, San Luis Obispo, CA 93407, USA}
\address[SJTU]{INPAC and School of Physics and Astronomy, Shanghai Jiao Tong University; Shanghai Laboratory for Particle Physics and Cosmology, Shanghai 200240, China}
\address[Yale]{Wright Laboratory, Department of Physics, Yale University, New Haven, CT 06520, USA}
\address[UNIZA]{Centro de Astropart\'iculas y Física de Altas Energ\'ias, Universidad de
Zaragoza, Zaragoza 50009, Spain}
\address[ARAID]{ARAID, Fundaci\'on Agencia Aragonesa para la Investigaci\'on y el
Desarrollo, Gobierno de Arag\'on, Zaragoza 50018, Spain}
\address[LBNLPhys]{Physics Division, Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
\address[BolognaAstro]{Dipartimento di Fisica e Astronomia, Alma Mater Studiorum -- Universit\`{a} di Bologna, Bologna I-40127, Italy}
\address[Saclay]{IRFU, CEA, Université Paris-Saclay, F-91191 Gif-sur-Yvette, France}
\address[LLNL]{Lawrence Livermore National Laboratory, Livermore, CA 94550, USA}
\address[BerkeleyNucEng]{Department of Nuclear Engineering, University of California, Berkeley, CA 94720, USA}
\address[Cassino]{Dipartimento di Ingegneria Civile e Meccanica, Universit\`{a} degli Studi di Cassino e del Lazio Meridionale, Cassino I-03043, Italy}
\address[JHU]{Department of Physics and Astronomy, The Johns Hopkins University, 3400 North Charles Street Baltimore, MD, 21211}
\address[INFNPadova]{INFN -- Sezione di Padova, Padova I-35131, Italy}
\address[LBNLEngineering]{Engineering Division, Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}
\address[AQUILA]{Dipartimento di Scienze Fisiche e Chimiche, Universit\`{a} dell’Aquila, L’Aquila I-67100, Italy}
\address[WISC]{Department of Physics, University of Wisconsin, Madison, Wisconsin 53706, USA}
\address[MatBerkely]{Department of Materials Science and Engineering, University of California, Berkeley, California 94720, USA}

\fntext[fn1]{Deceased}
\fntext[fn2]{Retired}

==> CUORE - PPNP_arXiv/cuore-authors_arXiv.tex <==
CUORE Collaboration: D. Q. Adams, C. Alduino, F. Alessandria, K. Alfonso, E. Andreotti, F. T. Avignone III, O. Azzolini, M. Balata, I. Bandac, T. I. Banks, G. Bari, M. Barucci, J. W. Beeman, F. Bellini, G. Benato, M. Beretta, A. Bersani, D. Biare, M. Biassoni, F. Bragazzi, A. Branca, C. Brofferio, A. Bryant, A. Buccheri, C. Bucci, C. Bulfon, A. Camacho, J. Camilleri, A. Caminata, A. Campani, L. Canonica, X. G. Cao, S. Capelli, M. Capodiferro, L. Cappelli, L. Cardani, M. Cariello, P. Carniti, M. Carrettoni, N. Casali, L. Cassina, E. Celi, R. Cereseto, G. Ceruti, A. Chiarini, D. Chiesa, N. Chott, M. Clemenza, D. Conventi, S. Copello, C. Cosmelli, O. Cremonesi, C. Crescentini, R. J. Creswick, J. S. Cushman, A. D'Addabbo, D. D'Aguanno, I. Dafinei, V. Datskov, C. J. Davis, F. Del Corso, S. Dell'Oro, M. M. Deninno, S. Di Domizio, V. Domp\`e, M. L. Di Vacri, L. Di Paolo, A. Drobizhev, L. Ejzak, R. Faccini, D. Q. Fang, G. Fantini, M. Faverzani, E. Ferri, F. Ferroni, E. Fiorini, M. A. Franceschi, S. J. Freedman, S. H. Fu, B. K. Fujikawa, R. Gaigher, S. Ghislandi, A. Giachero, L. Gironi, A. Giuliani, L. Gladstone, J. Goett, P. Gorla, C. Gotti, C. Guandalini, M. Guerzoni, M. Guetti, T. D. Gutierrez, E. E. Haller, K. Han, E. V. Hansen, K. M. Heeger, R. Hennings-Yeomans, K. P. Hickerson, R. G. Huang, H. Z. Huang, M. Iannone, L. Ioannucci, J. Johnston, R. Kadel, G. Keppel, L. Kogler, Yu. G. Kolomensky, A. Leder, C. Ligi, K. E. Lim, R. Liu, L. Ma, Y. G. Ma, C. Maiano, M. Maino, L. Marini, M. Martinez, C. Martinez Amaya, R. H. Maruyama, D. Mayer, R. Mazza, Y. Mei, N. Moggi, S. Morganti, P. J. Mosteiro, S. S. Nagorny, T. Napolitano, M. Nastasi, J. Nikkel, S. Nisi, C. Nones, E. B. Norman, V. Novati, A. Nucciotti, I. Nutini, T. O'Donnell, M. Olcese, E. Olivieri, F. Orio, D. Orlandi, J. L. Ouellet, S. Pagan, C. E. Pagliarone, L. Pagnanini, M. Pallavicini, V. Palmieri, L. Pattavina, M. Pavan, M. Pedretti, R. Pedrotta, A. Pelosi, M. Perego, G. Pessina, V. Pettinacci, G. Piperno, C. Pira, S. Pirro, S. Pozzi, E. Previtali, A. Puiu, S. Quitadamo, F. Reindl, F. Rimondi, L. Risegari, C. Rosenfeld, C. Rossi, C. Rusconi, M. Sakai, E. Sala , C. Salvioni, S. Sangiorgio, D. Santone, D. Schaeffer, B. Schmidt, J. Schmidt, N. D. Scielzo, V. Sharma, V. Singh, M. Sisti, A. R. Smith, D. Speller, F. Stivanello, P. T. Surukuchi, L. Taffarello, L. Tatananni, M. Tenconi, F. Terranova, M. Tessaro, C. Tomei, G. Ventura, K. J.  Vetter, M. Vignati, S. L. Wagaarachchi, J. Wallig, B. S. Wang, H. W. Wang, B. Welliver, J. Wilson, K. Wilson, L. A. Winslow, T. Wise, L. Zanotti, C. Zarra, G. Q. Zhang, B. X. Zhu, S. Zimmermann, S. Zucchelli

==> cuore-authors_arXiv.tex <==
CUORE Collaboration: D. Q. Adams, C. Alduino, F. Alessandria, K. Alfonso, E. Andreotti, F. T. Avignone III, O. Azzolini, M. Balata, I. Bandac, T. I. Banks, G. Bari, M. Barucci, J. W. Beeman, F. Bellini, G. Benato, M. Beretta, A. Bersani, D. Biare, M. Biassoni, F. Bragazzi, A. Branca, C. Brofferio, A. Bryant, A. Buccheri, C. Bucci, C. Bulfon, A. Camacho, J. Camilleri, A. Caminata, A. Campani, L. Canonica, X. G. Cao, S. Capelli, M. Capodiferro, L. Cappelli, L. Cardani, M. Cariello, P. Carniti, M. Carrettoni, N. Casali, L. Cassina, E. Celi, R. Cereseto, G. Ceruti, A. Chiarini, D. Chiesa, N. Chott, M. Clemenza, D. Conventi, S. Copello, C. Cosmelli, O. Cremonesi, C. Crescentini, R. J. Creswick, J. S. Cushman, A. D'Addabbo, D. D'Aguanno, I. Dafinei, V. Datskov, C. J. Davis, F. Del Corso, S. Dell'Oro, M. M. Deninno, S. Di Domizio, V. Domp\`e, M. L. Di Vacri, L. Di Paolo, A. Drobizhev, L. Ejzak, R. Faccini, D. Q. Fang, G. Fantini, M. Faverzani, E. Ferri, F. Ferroni, E. Fiorini, M. A. Franceschi, S. J. Freedman, S. H. Fu, B. K. Fujikawa, R. Gaigher, S. Ghislandi, A. Giachero, L. Gironi, A. Giuliani, L. Gladstone, J. Goett, P. Gorla, C. Gotti, C. Guandalini, M. Guerzoni, M. Guetti, T. D. Gutierrez, E. E. Haller, K. Han, E. V. Hansen, K. M. Heeger, R. Hennings-Yeomans, K. P. Hickerson, R. G. Huang, H. Z. Huang, M. Iannone, L. Ioannucci, J. Johnston, R. Kadel, G. Keppel, L. Kogler, Yu. G. Kolomensky, A. Leder, C. Ligi, K. E. Lim, R. Liu, L. Ma, Y. G. Ma, C. Maiano, M. Maino, L. Marini, M. Martinez, C. Martinez Amaya, R. H. Maruyama, D. Mayer, R. Mazza, Y. Mei, N. Moggi, S. Morganti, P. J. Mosteiro, S. S. Nagorny, T. Napolitano, M. Nastasi, J. Nikkel, S. Nisi, C. Nones, E. B. Norman, V. Novati, A. Nucciotti, I. Nutini, T. O'Donnell, M. Olcese, E. Olivieri, F. Orio, D. Orlandi, J. L. Ouellet, S. Pagan, C. E. Pagliarone, L. Pagnanini, M. Pallavicini, V. Palmieri, L. Pattavina, M. Pavan, M. Pedretti, R. Pedrotta, A. Pelosi, M. Perego, G. Pessina, V. Pettinacci, G. Piperno, C. Pira, S. Pirro, S. Pozzi, E. Previtali, A. Puiu, S. Quitadamo, F. Reindl, F. Rimondi, L. Risegari, C. Rosenfeld, C. Rossi, C. Rusconi, M. Sakai, E. Sala , C. Salvioni, S. Sangiorgio, D. Santone, D. Schaeffer, B. Schmidt, J. Schmidt, N. D. Scielzo, V. Sharma, V. Singh, M. Sisti, A. R. Smith, D. Speller, F. Stivanello, P. T. Surukuchi, L. Taffarello, L. Tatananni, M. Tenconi, F. Terranova, M. Tessaro, C. Tomei, G. Ventura, K. J.  Vetter, M. Vignati, S. L. Wagaarachchi, J. Wallig, B. S. Wang, H. W. Wang, B. Welliver, J. Wilson, K. Wilson, L. A. Winslow, T. Wise, L. Zanotti, C. Zarra, G. Q. Zhang, B. X. Zhu, S. Zimmermann, S. Zucchelli
